Normal Form Bisimulations By Value

Normal form bisimilarities are a natural form of program equivalence resting on open terms, first introduced by Sangiorgi in call-by-name. The literature contains a normal form bisimilarity for Plotkin's call-by-value $\lambda$-calculus, Lassen's \emph{enf bisimilarity}, which validates all of Moggi's monadic laws and can be extended to validate $\eta$. It does not validate, however, other relevant principles, such as the identification of meaningless terms -- validated instead by Sangiorgi's bisimilarity -- or the commutation of $\letexp$s. These shortcomings are due to issues with open terms of Plotkin's calculus. We introduce a new call-by-value normal form bisimilarity, deemed \emph{net bisimilarity}, closer in spirit to Sangiorgi's and satisfying the additional principles. We develop it on top of an existing formalism designed for dealing with open terms in call-by-value. It turns out that enf and net bisimilarities are \emph{incomparable}, as net bisimilarity does not validate Moggi's laws nor $\eta$. Moreover, there is no easy way to merge them. To better understand the situation, we provide an analysis of the rich range of possible call-by-value normal form bisimilarities, relating them to Ehrhard's relational model.

==> figures/RSC-lassen-for-naf.tex <==
% !TEX root = main.tex
\begin{tabular}{cccccc} 
%\textsc{Lassen's closure (for toy simulations)}
%\\[6pt]
\begin{tabular}{cccccc} 
	\infer[\sclift ]{\tmrone \lasrel \tmrtwo} {\tmrone \rel \tmrtwo}
	&
	\infer[\scvar]{\var \lasrel \var}	{}
	&
	\infer[\scabs ]{\la\var\tmrone \lasrel \la\var\tmrtwo} {\tmrone \lasrel \tmrtwo}
	&
		\infer[\scapp ] {\tmrone\tmrthree  \lasrel  \tmrtwo\tmrfour} {\tmrone  \lasrel \tmrtwo & \tmrthree \lasrel \tmrfour }  
\end{tabular}
\\[14pt]
\begin{tabular}{cccccc}
		\infer[\scesub ]{\tmrone\esub\var{\tmrthree} \lasrel \tmrtwo\esub\var{\tmrfour}{}} {\tmrone \lasrel \tmrtwo & \tmrthree \lasrel \tmrfour }
&
	\infer[\scsub ]{\tmrone\isub\var{\valp} \lasrel \tmrtwo\isub\var{\valptwo}{}} {\tmrone \lasrel \tmrtwo & \valp \lasrel \valptwo }	
\end{tabular}
\end{tabular}

==> figures/VSC-big-step-pratical-values.tex <==
% !TEX root = main.tex
\begin{tabular}{cccc}
	\begin{tabular}{c\colspace cc}
	\infer[(\bslasax)]{\val \bsw 0 \val}{}
	& 
	\infer[(\bslas?)]{\tm\tmtwo \bsw {k+h+i+1} \ntm}{
		\tm \bsw k \la\var\tmthree
		&
		\tmtwo \bsw h \val
		&
		{\tmthree\isub\var\val} \bsw i \ntm}
%	\\[10pt]
%	\infer[(\bslas?)]{\tm\tmtwo \bsw {k+h} \ntm\ntmtwo}{
%	\tm \bsw k \ntm \neq \la\var\tmthree
%	&
%	\tmtwo \bsw h \ntm
%	}
%	&
%	\infer[(\bslas?)]{\tm\tmtwo \bsw {k+h}(\la\var\tmthree)\ntm}{
%	\tm \bsw k \la\var\tmthree
%	&
%	\tmtwo \bsw h \ntm\neq\val
%	}} 
&\infer[(\bslas?)]{\tm\tmtwo \bsw {k+h} \ntmONE=\ntm\ntmtwo}{
	\tm \bsw k \ntm
	&
	\tmtwo \bsw h \ntmtwo}
	\end{tabular}
	\\[12pt]

%	&
%	\multicolumn{2}{c}{
%		\infer[(\bslas?)]{\tm\tmtwo \bsw {k+h}\ntm\ntmtwo}{
%			\tm \bsw k \ntm\neq\val
%			&
%			\tmtwo \bsw h \ntmtwo}}

\end{tabular}
